Position-dependent power spectrum: a new observable in the large-scale structure

We present a new observable, position-dependent power spectrum, to measure the large-scale structure bispectrum in the squeezed configuration, where one wavenumber is much smaller than the other two. The squeezed-limit bispectrum measures how the small-scale power spectrum is modulated by a long-wavelength overdensity, which is due to gravitational evolution and possibly inflationary physics. We divide a survey into small subvolumes, compute the local power spectrum and the mean overdensity in each subvolume, and measure the correlation between them. The correlation measures the integral of the bispectrum, which is dominated by squeezed configurations if the scale of the local power spectrum is much smaller than the subvolume size. We use the separate universe approach to model how the small-scale power spectrum is affected by a long-wavelength overdensity gravitationally. This models the nonlinearity of the bispectrum better than the perturbation theory approach. Not only the new observable is easy to interpret, but it sidesteps the complexity of the full bispectrum estimation as both power spectrum and mean overdensity are easier to estimate than the full bispectrum. We report on the first measurement of the position-dependent correlation function from the SDSS-III BOSS DR10 CMASS sample. We detect the bispectrum of the CMASS sample, and constrain their nonlinear bias combining with anisotropic clustering and weak lensing. We finally study the response of the small-scale power spectrum to 1-3 long-wavelength overdensities. We compare the separate universe approach to separate universe simulations to unprecedented accuracy. We test the standard perturbation theory (SPT) hypothesis that the nonlinear n-point function is fully predicted by the linear power spectrum at the same time. We find discrepancies on small scales, which suggest that SPT fails even if it is calculated to all orders.

==> lebenslauf.tex <==
\chapter*{Lebenslauf}

Sigmund Stintzing

\vspace*{2.0cm}

\begin{tabular}{ll}

Geburtsdatum & Geburt in Geburtsort \\[1.5ex]
Schulzeit & Besuch der Schule in Ort \\[1.5ex]
 ... & ...
\end{tabular}

